DU-VLG: Unifying Vision-and-Language Generation via Dual Sequence-to-Sequence Pre-training

Due to the limitations of the model structure and pre-training objectives, existing vision-and-language generation models cannot utilize pair-wise images and text through bi-directional generation. In this paper, we propose DU-VLG, a framework which unifies vision-and-language generation as sequence generation problems. DU-VLG is trained with novel dual pre-training tasks: multi-modal denoising autoencoder tasks and modality translation tasks. To bridge the gap between image understanding and generation, we further design a novel commitment loss. We compare pre-training objectives on image captioning and text-to-image generation datasets. Results show that DU-VLG yields better performance than variants trained with uni-directional generation objectives or the variant without the commitment loss. We also obtain higher scores compared to previous state-of-the-art systems on three vision-and-language generation tasks. In addition, human judges further confirm that our model generates real and relevant images as well as faithful and informative captions.

==> 010train_detail.tex <==

\section{Additional Training Details}

\subsection{Pre-training}

Following ViT, we use a patch size of $p=16$ for all the experiments. For VQ-VAE, we take the off-the-shelf VQ-GAN~\cite{Esser_2021_CVPR}, which is a variant of VQ-VAE. The VQ-GAN maps each $16 \times 16$ pixels as a discrete visual token, with a vocabulary size of $|\mathcal{V}| = 16384$.

For base and large model, we use \texttt{ViT-base} and \texttt{ViT-large} with a patch size of $p=16$ to extract image patch embeddings. ViT weights are set frozen during pre-training. Since image sequences are longer than text sequences, we set $\alpha = 0.05$ and $\beta=1$ for all experiments. For model optimization, we utilize Adam optimizer with a gradient clipping of 1.0 and a batch size equivalent of 1024. 

\subsection{Downstream Tasks}

\noindent
\textbf{Text-to-Image Generation.} The CUB dataset contains 200 bird categories with 11,788 images. Each image has ten text descriptions. We follow the standard split which uses 150 categories with 8,855 images for training and the remaining 50 categories with 2,933 images for testing. The COCO dataset contains 82,784 images for training and 40,505 for testing. Each image has five text descriptions.

We fine-tune on the pre-trained model with a learning rate of 1e-4 for 300 epoches on both datasets. Similar to ~\newcite{DBLP:journals/corr/abs-2102-12092}, we sample 16 images per caption with nucleus sampling strategy~\cite{Holtzman2020The}
During testing, we first sample 16 images per caption and rerank the generated images with a CLIP model~\cite{pmlr-v139-radford21a}. The CLIP model selects the best image based on its correlation with the text description. 

\noindent
\textbf{Image Captioning.} For COCO dataset, we follow the Karparthy split which has 113,287 images for training
, 5000 and 5000 images for training, validation and test. Each image has 5 human-written captions. During inference, we generate a caption for each image and evaluate against five references. 

We fine-tune on COCO dataset with a learning rate of 3e-5. 
Vision Transformer layers are trainable during fine-tuning. Following ~\newcite{10.1007/978-3-030-58577-8_8}, we add object labels detected by the object detection model as additional text inputs. We find object labels improve CIDER and BLEU scores for at least 1 point and 0.3 points. During testing, we use beam search with a beam size of 5.

\noindent
\textbf{Visual Commonsense Reasoning.} For visual commonsense reasoning, we fine-tune with a learning rate of 3e-5 and set vision transformer layers trainable. During testing, we use top-k sampling with $k=50$. We find top-k sampling yields more meaningful responses compared to beam search.


